A Study of Concurrency Bugs and Advanced Development Support for Actor-based Programs

The actor model is an attractive foundation for developing concurrent applications because actors are isolated concurrent entities that communicate through asynchronous messages and do not share state. Thereby, they avoid concurrency bugs such as data races, but are not immune to concurrency bugs in general. This study taxonomizes concurrency bugs in actor-based programs reported in literature. Furthermore, it analyzes the bugs to identify the patterns causing them as well as their observable behavior. Based on this taxonomy, we further analyze the literature and find that current approaches to static analysis and testing focus on communication deadlocks and message protocol violations. However, they do not provide solutions to identify livelocks and behavioral deadlocks. The insights obtained in this study can be used to improve debugging support for actor-based programs with new debugging techniques to identify the root cause of complex concurrency bugs.

==> Makefile <==
# This Makefile relies on LaTeX-Mk
# See: http://latex-mk.sourceforge.net/

NAME=paper

KNITR=$(wildcard sections/*.Rnw)
KNITR_TEX=$(KNITR:.Rnw=.tex)
KNITR_TEX=$(patsubst sections/%.Rnw,gen/%.tex,$(KNITR))
TEXSRCS=$(NAME).tex $(wildcard sections/*.tex) $(KNITR_TEX)
USE_PDFLATEX=true
BIBTEXSRCS=references.bib

CLEAN_FILES+=$(wildcard *.synctex.gz) $(wildcard *.fdb_latexmk) $(wildcard *.fls) $(KNITR_TEX)

ifeq ($(CI_SERVER),yes)
	GV=curl -F file=@$(NAME).pdf -F filename=$(NAME).pdf -F title="Latest Version" -F channels="\#writing" -F token=xoxb-141106319171-uuvspxaiUNcuDt7YeYZhWW11 https://slack.com/api/files.upload && touch 
else
	GV=@open -a Skim.app 
endif



gen/%.tex: sections/%.Rnw gen scripts/*.R
	scripts/knit.R $< $@

# We are going to try a couple of standard locations to find LaTeX-Mk:
-include ~/.local/share/latex-mk/latex.gmk
-include /usr/local/share/latex-mk/latex.gmk
-include /opt/local/share/latex-mk/latex.gmk
-include /usr/share/latex-mk/latex.gmk

gen:
	-mkdir gen

open:
	mate $(TEXSRCS)

clobber: clean
	rm -Rf gen cache

html5:
	-mkdir tmp-html
	~/Projects/misc/latex-to-html5/ht-latex fast.tex tmp-html

